Conversational Neuro-Symbolic Commonsense Reasoning

In order for conversational AI systems to hold more natural and broad-ranging conversations, they will require much more commonsense, including the ability to identify unstated presumptions of their conversational partners. For example, in the command "If it snows at night then wake me up early because I don't want to be late for work" the speaker relies on commonsense reasoning of the listener to infer the implicit presumption that they wish to be woken only if it snows enough to cause traffic slowdowns. We consider here the problem of understanding such imprecisely stated natural language commands given in the form of "if-(state), then-(action), because-(goal)" statements. More precisely, we consider the problem of identifying the unstated presumptions of the speaker that allow the requested action to achieve the desired goal from the given state (perhaps elaborated by making the implicit presumptions explicit). We release a benchmark data set for this task, collected from humans and annotated with commonsense presumptions. We present a neuro-symbolic theorem prover that extracts multi-hop reasoning chains, and apply it to this problem. Furthermore, to accommodate the reality that current AI commonsense systems lack full coverage, we also present an interactive conversational framework built on our neuro-symbolic system, that conversationally evokes commonsense knowledge from humans to complete its reasoning chains.

==> COMET_generations.tex <==
\subsection*{COMET generations}

COMET goal generations:
\begin{itemize}
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to clear the air
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to be safe
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to be unpredictable
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to show off
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to forecast
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to prepare
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to have a good time
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to prepare for a storm
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to have a good experience
\item IF there are thunderstorms in the forecast within a few hours THEN remind me to close the windows BECAUSE I WANT to make sure everything is safe
\end{itemize}

COMET action generations:
\begin{itemize}
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to enjoy the weather BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to be safe BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to have fun BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to take pictures BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to take a break BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to have a good time BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to relax BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to enjoy a good time BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to go to the store BECAUSE i want to keep my home dry.
\item IF there are thunderstorms in the forecast within a few hours THEN I WANT to make sure everything is fine BECAUSE i want to keep my home dry.
\end{itemize}

==> boarder_impacts.tex <==
\section*{Broader Impact}
Performing successful commonsense reasoning is dependent on having a large knowledge base of commonsense facts.
% Commonsense reasoning relies on a knowledge base (KB) of commonsense facts, but 
However, there is currently no technology that has the capacity to store the sum total of all human knowledge.
% one has access to a KB that is large enough to do commonsense with, 
Therefore, we propose to conversationally complete knowledge bases by interacting with humans. Learning through conversational interactions is a research direction that can impact the machine learning community and can be combined with many learning algorithms to address issues with data sparsity. 
Moreover, it is expected for a future version of Siri or Google home or any other smart phone/home assistant to be equipped with this type of interaction strategy, so that they can build more personalized beliefs about their users. Therefore, leveraging conversational interactions for learning is a plausible opportunity. However, as is the case with any model that collects user information, this collected data could be susceptible to attacks or privacy breach.

The importance of commonsense reasoning and its lack of it in current AI systems is a known impediment to having truly intelligent systems \cite{davis2015commonsense}. Therefore, this research is an attempt towards taking the literature on commonsense reasoning a small step forward 
by proposing a new unstudied aspect of commonsense reasoning which is to attempt to explicitly uncover unspoken commonsense presumptions from a given natural language utterance.
% commonsense reasoning benchmark and a novel commonsense reasoning engine. %and can benefit many applications in natural language understanding, machine translation, computer vision and robotics.
% Commonsense reasoning remains an unsolved problem at the heart of AI. This paper proposes an open direction for research in commonsense reasoning and
% proposes . 
This can be further extended to benchmarks that uncover presumptions given an image of a scene, to uncover objects that are presumably in the photo but are not shown. For example, to presume that in an image of a room there exists a wall hook that supports a frame on the wall.

% For example, consider showing a human a photo of a dining room. They would immediately presume that there must be a table underneath the table-cloth or that the objects hanging on the wall are presumably supported by hooks and many more [example taken from \cite{davis2015commonsense}]. This can also be extended to explicitly uncover presumptions while watching a movie. %\facomment{consider replacing the example with an example in your own words}
One of the immediate impacts of this work is to make AI assistants that can engage in natural sounding conversations with humans. In order to be good at conversation, computers should be able to make presumptions driven by common sense about an input statement. If solved, we would have conversational agents that sound smarter to humans. We propose a neuro-symbolic reasoning engine that aims to address this problem.
% Another impact of this work is in proposing a neuro-symbolic solution for the proposed commonsense reasoning problem.

==> introduction.tex <==
\section{Introduction}
Justice et al. \cite{justiceguide} state in their book that ``Children develop their knowledge of the world around them as they interact with their environment directly and indirectly. The direct experiences children have in their homes, schools and communities certainly provide the greatest amount of input to the world knowledge base.''. This knowledge arises from both physical and conversational interactions. In this paper, we test the hypothesis that just like a human child, machines need interaction to acquire world knowledge and develop commonsense reasoning abilities, and we study the effect of conversational interactions on this knowledge acquisition. Most of the literature on commonsense reasoning 
relies %rely [kmm- most-> relies]
on extracting the largest possible snapshot of 
%the [kmm- removed]
world knowledge and either 
query %query [kmm- on-> extracting and querying]
it or 
propose %propose [kmm- most-> proposes][could also parse as 'relies on-> proposing' or 'querying or proposing', may be better to restructure the sentence][fa- it was the later, so i restructured]
automated knowledge base completion methods for it. We argue that it is necessary to equip reasoning engines with an interaction strategy facilitating the extraction of just-in-time information needed for reasoning. 
%, through conversation with a human user [kmm- removed; conversation is covered by 'interaction' earlier in the sentence]
In this paper, we 
take up %take a few steps towards [kmm- rephrase (take steps/take steps repetitive)]
this grand goal, %[kmm- comma added]
and although we do not solve the whole challenge, we take the first steps needed for addressing it. 
Specifically, here we propose a ``soft'' commonsense reasoning engine and solve targeted knowledge base completion problems based on the information provided by the user through a conversational interface.

% We state this as our overarching grand research goal and mention carefully that we are taking a few steps towards this grand goal. Although it does not solve all of it but it is a step towards achieving this goal. This is just a first step however its a part of a very well reasoned and ambitious project. Then we also carefully describe the limitations of the project
% In other words, our overarching goal is having a human construct a reasoning system that does not have commonsense and extract commonsense from the user through conversation.
% \amoscomment{I think that it might be better saying something like: this work takes the first step towards ... I think that the paper could also benefit from adding a few sentences at the beginning.} \facomment{Is this resolved now?}

We believe that this is the right time for this proposal specifically since conversational agents such as Siri, Google home, Alexa and Cortana among others are starting to enter our daily lives. Therefore, it is plausible to assume that 
such agents %we [kmm- rephrase]
have access to conversation with a human for extracting commonsense knowledge. In this paper, we work with the Learning by Instruction Agent (LIA) \citep{azaria2016instructable,labutov2018lia} and develop a commonsense reasoning system for her called CORGI (\textbf{CO}mmonsense \textbf{R}easonin\textbf{G} by \textbf{I}nstruction). In what follows, we present our definition of commonsense reasoning for LIA after briefly introducing her. % It is worth noting, however, that the proposed method is not limited to a specific conversational agent. 
% \kmcomment{Anthropomorphizing LIA (referring to the agent as 'her') is a somewhat political choice -- it's okay to make it, but make it consciously.}

LIA is an intelligent agent that operates on 
a user's smartphone. %the phone [kmm- rephrase (you do not call LIA; there are other agents where you call in so it's important to make the distinction)]
%and can be taught new commands through user instructions. [kmm- removed (covered in the very next sentence)]
End users add new functionalities to LIA through verbal instructions and teach her how to perform new tasks. For example, the user can tell LIA, ``whenever it snows at night, wake me up 30 minutes early''. If LIA does not understand how to perform this task, she will ask the user to instruct her by breaking the task down into a set of steps in a teaching session. In this case, the user can say, ``(first) open the weather app, (second) see if the night weather condition is snow, (third) if true then adjust my alarm to 30 minutes earlier''. After this teaching session, LIA can perform this task. 

One phenomenon we have noticed in collecting these types of ``Whenever $S$ occurs, then do $A$'' instructions is that people often {\em underspecify} the precondition $S$. For example, one instructor might want to wake up early when it snows because they are concerned about getting to work on time.  For this user, the implied precondition is not really ``whenever it snows,'' but instead ``whenever it snows enough to cause traffic slowdowns, and it's a workday.'' The point is %Amos: I think that "the point is" doesn't sound good. How about "Naturally,"?
that people often fail to specify  such detailed conditions, perhaps because they are used to speaking to other people who possess the common sense needed to infer the more specific intent of the speaker.

Our goal for LIA is to use background commonsense knowledge to reason about the user's more specific intent, and to discuss this with the user in order to create the correct preconditions for the recommended action.  Therefore, we assume LIA can obtain statements from the user that fit the logical template ``Whenever $S$ occurs, do $A$ because I want to achieve goal $G$.''\footnote{Note in LIA's conversational setting, if the user gives an instruction of the form ``Whenever $S$ occurs, do $A$.'' and omits the reason, then LIA can simply respond ``Why do you want to do that?'' in order to prompt for the missing reason $G$.}
%LIA then generalizes from this statement to other actions. For example, if the user says, ``if the weather is rainy tomorrow then set an alarm for 1 hour later'', LIA can perform this action without needing to be taught again. However, this generalization has some limitations which 
%stem %stems [kmm- limitations->stem]
%from the lack of reasoning capabilities in LIA. 
For example consider the following two statements: %, [kmm- colon replaces comma]
\begin{itemize}
\item Whenever it snows at night, wake me up 30 minutes early because I don't want to be late to work
\item Whenever it snows at night, wake me up 30 minutes early because I have never seen the snow before 
\end{itemize}
Note that in the first statement, the user will not want to wake up early on a weekend or a holiday (assuming that they do not work then) whereas in the second scenario, the user will want to wake up early regardless of the date in order to see snow for the first time -- but might not want to wake up early once she has seen snow for the first time.

In CORGI, the role of commonsense reasoning is to derive the intended condition to use in place of the stated $S$ given an ``If $S$ then do $A$ because $G$'' statement from the user. Its general approach is to derive an explanation of how action $A$, performed in state $S$ will achieve goal $G$, and then to derive the intended precondition $S$ by collecting the preconditions on $S$ that allow this explanation to hold.  CORGI has access to a limited amount of general background knowledge about the world, represented in a logic programming language. Reasoning reduces to using this background knowledge to perform multi-hop logical inference. If no reasoning path is found, CORGI initiates a conversation with the user to extract relevant background knowledge and adds it to its underlying understanding of the world.  This newly acquired background knowledge will be used in future user interactions with CORGI. In essence, we are performing knowledge base completion through conversation, on a need-driven basis. Note that in earlier work Hixon et al. \cite{hixon2015learning} perform relation extraction using human interaction for question answering. Although the general idea of using human interaction is similar to our proposal, the information extraction method and the problem studied in \cite{hixon2015learning} differs from our setting. To the best of our knowledge, CORGI is the first conversational assistant that targets completing reasoning paths.
% \amoscomment{'their' seems like a typo, not sure what you are saying} --> resolved
% Therefore, our reasoning system is a commonsense reasoning by instruction engine. 

% \amoscomment{I find it hard to understand when 'LIA' refers to the agent from previous work, and when it refers to new capabilities added by this work.} \facomment{is this resolved now, Amos?} %Yes, Thanks!

% In this paper we develop a reasoning system for LIA that is capable of commonsense reasoning in order to generalize correctly given if-then user commands through the because statement.

CORGI's main reasoning component is the multi-hop inference system. Since the knowledge is represented in a logic programming language, the underlying inference algorithm is backward chaining. However, backward chaining in its traditional form is not robust to variations in natural language. This is specifically of importance since CORGI allows open-domain dialog with the user
to reduce the startup cost of the user having to learn a %so that the user is not limited to a [kmm- is this rephrase correct?]
specific grammar or vocabulary. Therefore, there is no parsing algorithm to resolve these variations. For example, in 
%the [kmm- removed]
traditional backward chaining, the statements ``if the forecast is snow tonight'' and ``if the weather is snowy tonight'' are thought of as two different statements whereas we want them both to map to the same representation. In order to address this, we propose a ``soft backward chaining'' algorithm that learns continuous representations or embeddings of the logical statements in the background knowledge. This will allow CORGI to indicate the equivalence of semantically similar statements based on the distance of their learned representations in the vector space. This soft backward chaining allows us to bridge a gap between symbolic AI and neural approaches using the best of both worlds.

% CORGI's soft backward chaining algorithm is end-to-end differentiable and is trained by looking at the proof traces of similar 

% kmm: resolve AA's confusion here with "compatible with deep-learning techniques"

% . This multi-hop reasoning system is end-to-end differentiable and supports soft multi-hop reasoning to account for natural language variations. \amoscomment{I might be missing something, but what does it mean being end-to-end differentiable, are you referring to differentiable functions (those that have a derivative), is this required in order to train the system? Or do you mean that the system obtains knowledge piece by piece. I guess you mean the former, but I did struggle with this.}

% \tmcomment{There are two main themes: 1. claiming that the reasoning can help get the generalization right, 2. how to do the reasoning in a way that is correct}

% \tmcomment{why are we doing reasoning this way and how can we make sure we can do it successfully. we need to compare it with the approximate inference and probabilistic inference methods for performing reasoning}

% \tmcomment{Our contributions are two fold. one is that we are proposing a reasoning strategy through conversation and are proposing to extract the missing information just in time to perform the correct reasoning. No one has the capacity to store the world's largest kb and until now everyone has tries to maintain the largest knowledge bases that there are. However, we are proposing a new way of doing this and it is to extract the correct part of the missing knowledge from the user. This is our grand goal and we have performed a set of small steps towards it... [layout the steps]. Another contribution is the soft unification part. In order to make this work we need to combine symbolic AI with neural approaches to bridge the gap and use the best of both worlds.}

% \tmcomment{reviewer question: How do we know if our method scales? No one has a large enough knowledge base that contains all the information there is in the world. And currently everyone in the field is trying to do this. However, we are proposing a method for extracting the right information just in time needed to perform the reasoning}

% \tmcomment{We do not know the user will give us the right answer even if we ask the right question} \kmcomment{Focus less on ``right'' answer/question here; there are many-to-many possible question/answer pairs that will give a good result. Make a definition of what success means in this context.}

% \tmcomment{Our goal is to have a conversation with the user and the main goal is to have the user give us the missing part of the information and in a funny/not so funny way this is a feature of the system}

% \tmcomment{consider the problem of learning procedures including triggers by conversation. When humans give instructions they are imprecise. In this project we are interested in having the human construct a reasoning system that does not have the commonsense and we want to use conversation to extract the commonsense from the user. We state this as our overarching grand research goal and mention carefully that we are taking a few steps towards this grand goal. Although it does not solve all of it but it is a step towards achieving this goal. This is just a first step however its a part of a very well reasoned and ambitious project. Then we also carefully describe the limitations of the project.}
